Colouring Digraphs

The aim of this thesis is to investigate how the structure of a digraph affects its dichromatic number and to extend various results on undirected colouring to digraphs. In the first part of this thesis, we examine how the dichromatic number interacts with other metrics. First, we consider the degree, which is the maximum number of neighbours of a vertex. In the undirected case, this corresponds to Brooks' theorem, a celebrated theorem with multiple variations and generalizations. In the directed case, there is no natural metric corresponding to the maximum degree, so we explore how different notions of maximum directed degree lead to either Brooks-like theorems or impossibility results. We also investigate the maximum local-arc connectivity, a metric that encompasses several degree-like metrics. The second part of this manuscript focuses on a directed analogue of the Gy\'arf\'as-Sumner conjecture. The Gy\'arf\'as-Sumner conjecture tries to characterize sets S of undirected graphs such that graphs with large enough chromatic number must contain a graph of S. This conjecture is still largely open. On digraphs, a corresponding conjecture was proposed by Aboulker, Charbit, and Naserasr. We prove several subcases of this conjecture, mainly demonstrating that certain classes of digraphs have bounded dichromatic number. In the last part of this thesis, we address the d-edge-defective-colouring problem, which involves colouring edges of a multigraph such that, for any vertex, no colour appears on more than d of its incident edges. When d equals one, this corresponds to the infamous edge-colouring problem. Shannon established a tight bound on the number of colours needed relative to the maximum degree when d equals one, and we extend this result to any value of d. We also explore this problem on simple graphs and prove results that extend Vizing's theorem to any value of d.

==> FrontBackMatter/Abstract.tex <==
% Abstract

%\renewcommand{\abstractname}{Abstract} % Uncomment to change the name of the abstract

\pdfbookmark[1]{Abstract}{Abstract} % Bookmark name visible in a PDF viewer

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax

\chapter*{Abstract}
Short summary of the contents\dots a great guide by 
Kent Beck how to write good abstracts can be found here:  
\begin{center}
\url{https://plg.uwaterloo.ca/~migod/research/beckOOPSLA.html}
\end{center}

\endgroup			

\vfill

==> FrontBackMatter/Declaration.tex <==
% Declaration

\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration} % Bookmark name visible in a PDF viewer

\chapter*{Declaration} % Declaration section text

\thispagestyle{empty}

Put your declaration here.
\bigskip
 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
\begin{tabular}{m{5cm}}
\\ \hline
\centering\myName \\
\end{tabular}
\end{flushright}


==> FrontBackMatter/Dedication.tex <==
% Dedication

\thispagestyle{empty}
\refstepcounter{dummy}

\pdfbookmark[1]{Dedication}{Dedication} % Bookmark name visible in a PDF viewer

\vspace*{3cm}

\begin{center}
\emph{Ohana} means family. \\
Family means nobody gets left behind, or forgotten. \\ \medskip
--- Lilo \& Stitch    
\end{center}

\medskip

\begin{center}
Dedicated to the loving memory of Rudolf Miede. \\ \smallskip
1939\,--\,2005
\end{center}

==> FrontBackMatter/Titlepage4.tex <==
% Title Page

\begin{titlepage}

\vspace*{-4.5cm}\hspace*{12.7cm}\includegraphics[scale=0.17]{upccropped.png}
\vspace*{1cm}

\begin{addmargin}[-1cm]{-2cm}


\begin{center}
\large

\vspace{-3cm}

{\large Université Paris-Cité}

École Doctorale de Sciences Mathématiques \\
de Paris Centre\\
{\small ED 386}\\


\vspace{0.5cm}
Préparée à l'\textbf{I}nstitut de \textbf{R}echerche \\
en \textbf{I}nformatique \textbf{F}ondamentale\\


\vspace{0.8cm}
\begingroup
\huge\color{Maroon}\spacedallcaps{\myTitle} \\  % Thesis title
\endgroup

\vspace{0.8cm}

Par \spacedlowsmallcaps{\myName}

\vspace{0.8cm}
    
{\Large Thèse de doctorat en Informatique}

\vspace{0.8cm}


Dirigée par \spacedlowsmallcaps{Pierre Charbit}


\vspace{0.5cm}

Présentée et soutenue publiquement\\
le \spacedlowsmallcaps{20/06/2023}




%\includegraphics[width=6cm]{gfx/TFZsuperellipse_bw} \\ \medskip % Picture

%\mySubtitle \\ \medskip % Thesis subtitle

%\myDegree \\
%\myDepartment \\
%\myFaculty \\
%\myUni \\ \bigskip

%\myTime\ -- \myVersion % Time and version
\end{center}

\vspace{0.7cm}

Devant un jury composé de :

\vspace{-0.2cm}

\begin{tabular}{p{13cm}p{5cm}}
        \multirow{2}{*}{\spacedlowsmallcaps{Pierre Charbit}} & \multirow{2}{*}{\emph{Directeur de thèse}} \\
       {\footnotesize Maître de conférences, Université Paris-Cité} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Pierre Aboulker}} & \multirow{2}{*}{\emph{Co-encadrant}} \\
       {\footnotesize Maître de conférences, École Normale Supérieure} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Stéphane Bessy}} & \multirow{2}{*}{\emph{Rapporteur}} \\
       {\footnotesize Professeur, Université de Montpellier} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Alexander Scott}} & \multirow{2}{*}{\emph{Rapporteur}} \\
       {\footnotesize Professeur, Université d'Oxford} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Marthe Bonamy}} & \multirow{2}{*}{\emph{Examinatrice}} \\
       {\footnotesize Chercheuse, CNRS, Université de Bordeaux} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Vincent Cohen-Addad}} & \multirow{2}{*}{\emph{Examinateur}} \\
       {\footnotesize Chercheur, Google Research} & \\[-0.4cm]
        \multirow{2}{*}{\spacedlowsmallcaps{Mat\v{e}j Stehlík}} & \multirow{2}{*}{\emph{Examinateur}} \\
       {\footnotesize Professeur, Université Paris-Cité} & \\[-0.4cm]
    
\end{tabular}
\end{addmargin}

\end{titlepage}
